Self-Supervised Velocity Estimation for Automotive Radar Object Detection Networks

This paper presents a method to learn the Cartesian velocity of objects using an object detection network on automotive radar data. The proposed method is self-supervised in terms of generating its own training signal for the velocities. Labels are only required for single-frame, oriented bounding boxes (OBBs). Labels for the Cartesian velocities or contiguous sequences, which are expensive to obtain, are not required. The general idea is to pre-train an object detection network without velocities using single-frame OBB labels, and then exploit the network's OBB predictions on unlabelled data for velocity training. In detail, the network's OBB predictions of the unlabelled frames are updated to the timestamp of a labelled frame using the predicted velocities and the distances between the updated OBBs of the unlabelled frame and the OBB predictions of the labelled frame are used to generate a self-supervised training signal for the velocities. The detection network architecture is extended by a module to account for the temporal relation of multiple scans and a module to represent the radars' radial velocity measurements explicitly. A two-step approach of first training only OBB detection, followed by training OBB detection and velocities is used. Further, a pre-training with pseudo-labels generated from radar radial velocity measurements bootstraps the self-supervised method of this paper. Experiments on the publicly available nuScenes dataset show that the proposed method almost reaches the velocity estimation performance of a fully supervised training, but does not require expensive velocity labels. Furthermore, we outperform a baseline method which uses only radial velocity measurements as labels.

==> figures/network_architecture.tex <==
\begin{tikzpicture}[scale=.9,every node/.style={minimum size=1},on grid]

\node (pointcloud) at (0,0) {\rotatebox{90}{pointcloud}};


%%% GNN %%%
\node (graphconstruction) [shift={($(pointcloud.east)+(1,1.2)$)}, draw, rounded corners] {graph construction};

\begin{scope}[local bounding box=gnn1,shift={($(pointcloud.east)+(.5,0)$)}]
% opacity to prevent graphical interference
\fill[white,fill opacity=0.9] (-.1,-.6) rectangle (.1,.6);
\draw[step=.2, black, shift={(-.1,0)}] (0,-.6) grid (.2,.6); %defining grids
\draw[black,very thick] (-.1,-.6) rectangle (.1,.6);%marking borders
\end{scope}

\begin{scope}[local bounding box=gnn2,shift={($(gnn1.east)+(.5,0)$)}]
% opacity to prevent graphical interference
\fill[white,fill opacity=0.9] (-.1,-.6) rectangle (.1,.6);
\draw[step=.2, black, shift={(-.1,0)}] (0,-.6) grid (.2,.6); %defining grids
\draw[black,very thick] (-.1,-.6) rectangle (.1,.6);%marking borders
\end{scope}

\begin{scope}[local bounding box=gnn3,shift={($(gnn2.east)+(.5,0)$)}]
% opacity to prevent graphical interference
\fill[white,fill opacity=0.9] (-.1,-.6) rectangle (.1,.6);
\fill[red] (-0.1,0.6) rectangle (0.1,0.4); \coordinate (point1) at (0.1,0.5);
\fill[blue] (-0.1,0.4) rectangle (0.1,0.2); \coordinate (point2) at (0.1,0.3);
\fill[orange] (-0.1,0.2) rectangle (0.1,0.0); \coordinate (point3) at (0.1,0.1);
\fill[red!50!white] (-0.1,0.0) rectangle (0.1,-0.2); \coordinate (point4) at (0.1,-0.1);
\fill[blue!50!white] (-0.1,-0.2) rectangle (0.1,-0.4); \coordinate (point5) at (0.1,-0.3);
\fill[orange!50!white] (-0.1,-0.4) rectangle (0.1,-0.6); \coordinate (point6) at (0.1,-0.5);
\draw[step=.2, black, shift={(-.1,0)}] (0,-.6) grid (.2,.6); %defining grids
\draw[black,very thick] (-.1,-.6) rectangle (.1,.6);%marking borders
\end{scope}

\node [below of=gnn2] {GNN layers};

\draw [-{stealth[length=3mm]}] (pointcloud) -- (gnn1);
\draw [-{stealth[length=3mm]}] (gnn1) -- (gnn2);
\draw [-{stealth[length=3mm]}] (gnn2) -- (gnn3);
\draw [-{stealth[length=3mm]}, rounded corners=2pt] (pointcloud) -- (graphconstruction.200);
\draw [-{stealth[length=3mm]}] (graphconstruction.south) -| (gnn1);
\draw [-{stealth[length=3mm]}] (graphconstruction.south) -| (gnn2);
\draw [-{stealth[length=3mm]}] (graphconstruction.south) -| (gnn3);

%%% Grid rendering %%%

\begin{scope}[local bounding box=gridrender,shift={($(gnn3.east)+(3,0)$)}, every node/.append style={
		yslant=0.5,xslant=-1},yslant=0.5,xslant=-1
	]
	% opacity to prevent graphical interference
	\fill[white,fill opacity=0.9] (-1,-1) rectangle (1,1);
	\draw[step=.2, black] (-1,-1) grid (1,1); %defining grids
	%\draw[step=1mm, red!50,thin] (3,1) grid (4,2);  %Nested Grid
	\draw[black,very thick] (-1,-1) rectangle (1,1);%marking borders
	\fill[red] (0.6,0.6) rectangle (0.4,0.4); \coordinate (gridcell1) at (0.5,0.5);
	\fill[blue] (-0.2,0.2) rectangle (-0.4,0.0); \coordinate (gridcell2) at (-0.3,0.1);
	\fill[orange] (-0.4,-0.6) rectangle (-0.6,-0.8); \coordinate (gridcell3) at (-0.5,-0.7);
	\fill[red!50!white] (-0.2,0.0) rectangle (0.0,0.2); \coordinate (gridcell4) at (-0.1,0.1);
	\fill[blue!50!white] (0.2,-0.8) rectangle (0.0,-1.0); \coordinate (gridcell5) at (0.1,-0.9);
	\fill[orange!50!white] (0.0,-0.2) rectangle (-0.2,0.0);  \coordinate (gridcell6) at (-0.1,-0.1);
	%Idem as above, for the n-th grid:
\end{scope}
\node [below = .1 of gridrender.south] {grid rendering};

\draw [-{stealth[length=3mm]}, rounded corners=2pt] (point1) -- (gridcell1);
\draw [-{stealth[length=3mm]}, rounded corners=2pt] (point2) -| (gridcell2);
\draw [-{stealth[length=3mm]}, rounded corners=2pt] (point3) -| (gridcell3);
\draw [-{stealth[length=3mm]}, rounded corners=2pt] (point4) -| (gridcell4);
\draw [-{stealth[length=3mm]}, rounded corners=2pt] (point5) -| (gridcell5);
\draw [-{stealth[length=3mm]}, rounded corners=2pt] (point6) -| (gridcell6);

%%% ResNet %%%
\node (stem) [below right = 1 and 2.5 of gridrender, draw, rounded corners] {stem};

\begin{scope}[local bounding box=resgrid1,shift={($(stem.east)+(2.2,0)$)}, every node/.append style={
	yslant=0,xslant=1},yslant=0,xslant=1
]
\fill[white,fill opacity=0.9] (-1,-.4) rectangle (1,.4);
\draw[black,very thick] (-1,-.4) rectangle (1,.4);%marking borders
\end{scope}

\node (res2) [above = .7 of resgrid1, draw, rounded corners] {ResNet block 2};
\node (res2_num) [circle,draw=black, fill=black, text=white, inner sep=0pt,minimum size=5pt] at ($(res2.west)-(0.2,0)$) {$\mathbf{3\times}$};

\begin{scope}[local bounding box=resgrid2,shift={($(res2.north)+(0,.5)$)}, every node/.append style={
	yslant=0,xslant=1},yslant=0,xslant=1
]
\fill[white,fill opacity=0.9] (-.8,-.32) rectangle (.8,.32);
\draw[black,very thick] (-.8,-.32) rectangle (.8,.32);%marking borders
\end{scope}

\node (res3) [above = .7 of resgrid2, draw, rounded corners] {ResNet block 3};
\node (res3_num) [circle,draw=black, fill=black, text=white, inner sep=0pt,minimum size=5pt] at ($(res3.west)-(0.2,0)$) {$\mathbf{6\times}$};

\begin{scope}[local bounding box=resgrid3,shift={($(res3.north)+(0,.4)$)}, every node/.append style={
	yslant=0,xslant=1},yslant=0,xslant=1
]
\fill[white,fill opacity=0.9] (-.6,-.24) rectangle (.6,.24);
\draw[black,very thick] (-.6,-.24) rectangle (.6,.24);%marking borders
\end{scope}

\node (res4) [above = .7 of resgrid3, draw, rounded corners] {ResNet block 4};
\node (res4_num) [circle,draw=black, fill=black, text=white, inner sep=0pt,minimum size=5pt] at ($(res4.west)-(0.2,0)$) {$\mathbf{6\times}$};

\begin{scope}[local bounding box=resgrid4,shift={($(res4.north)+(0,.3)$)}, every node/.append style={
	yslant=0,xslant=1},yslant=0,xslant=1
]
\fill[white,fill opacity=0.9] (-.4,-.16) rectangle (.4,.16);
\draw[black,very thick] (-.4,-.16) rectangle (.4,.16);%marking borders
\end{scope}

\node (res5) [above = .7 of resgrid4, draw, rounded corners] {ResNet block 5};
\node (res5_num) [circle,draw=black, fill=black, text=white, inner sep=0pt,minimum size=5pt] at ($(res5.west)-(0.2,0)$) {$\mathbf{3\times}$};

\begin{scope}[local bounding box=resgrid5,shift={($(res5.north)+(0,.3)$)}, every node/.append style={
	yslant=0,xslant=1},yslant=0,xslant=1
]
\fill[white,fill opacity=0.9] (-.25,-.1) rectangle (.25,.1);
\draw[black,very thick] (-.25,-.1) rectangle (.25,.1);%marking borders
\end{scope}

\begin{scope}[local bounding box=conv_resfpn,shift={($(resgrid5.east)+(1.2, 0)$)}, every node/.append style={
	yslant=.5,xslant=0,solid},yslant=.5,xslant=0,solid
]
\fill[white,fill opacity=0.9] (-.08,-.2) rectangle (.08,.2);
\draw[black,very thick] (-.08,-.2) rectangle (.08,.2);%marking borders
\end{scope}
\node [below right = .4 and .5 of conv_resfpn] {\footnotesize $1\times1$ conv};

\draw [-{stealth[length=3mm]}, rounded corners=3pt] (gridrender) -| (stem);
\draw [-{stealth[length=3mm]}] (stem) -- (resgrid1);
\draw [-{stealth[length=3mm]}] (resgrid1) -- (res2);
\draw [-{stealth[length=3mm]}] (res2) -- (resgrid2);
\draw [-{stealth[length=3mm]}] (resgrid2) -- (res3);
\draw [-{stealth[length=3mm]}] (res3) -- (resgrid3);
\draw [-{stealth[length=3mm]}] (resgrid3) -- (res4);
\draw [-{stealth[length=3mm]}] (res4) -- (resgrid4);
\draw [-{stealth[length=3mm]}] (resgrid4) -- (res5);
\draw [-{stealth[length=3mm]}] (res5) -- (resgrid5);
\draw [-{stealth[length=3mm]}] (resgrid5) -- (conv_resfpn);

%%% FPN part %%%
\node (fpn4) [right = 2.5 of resgrid4, draw, rounded corners] {FPN block 4};
\begin{scope}[local bounding box=fpngrid4,shift={($(fpn4.south)-(0,.3)$)}, every node/.append style={
	yslant=0,xslant=1},yslant=0,xslant=1
]
\fill[white,fill opacity=0.9] (-.4,-.16) rectangle (.4,.16);
\draw[black,very thick] (-.4,-.16) rectangle (.4,.16);%marking borders
\end{scope}

\node (fpn3) [right = 2.5 of resgrid3, draw, rounded corners] {FPN block 3};
\begin{scope}[local bounding box=fpngrid3,shift={($(fpn3.south)-(0,.4)$)}, every node/.append style={
	yslant=0,xslant=1},yslant=0,xslant=1
]
\fill[white,fill opacity=0.9] (-.6,-.24) rectangle (.6,.24);
\draw[black,very thick] (-.6,-.24) rectangle (.6,.24);%marking borders
\end{scope}

\node (fpn2) [right = 2.5 of resgrid2, draw, rounded corners] {FPN block 2};
\begin{scope}[local bounding box=fpngrid2,shift={($(fpn2.south)-(0,.5)$)}, every node/.append style={
	yslant=0,xslant=1},yslant=0,xslant=1
]
\fill[white,fill opacity=0.9] (-.8,-.32) rectangle (.8,.32);
\draw[black,very thick] (-.8,-.32) rectangle (.8,.32);%marking borders
\end{scope}

\draw [-{stealth[length=3mm]}, rounded corners=3pt] (conv_resfpn) -| (fpn4);
\draw [-{stealth[length=3mm]}] (fpn4) -- (fpngrid4);
\draw [-{stealth[length=3mm]}] (fpngrid4) -- (fpn3);
\draw [-{stealth[length=3mm]}] (fpn3) -- (fpngrid3);
\draw [-{stealth[length=3mm]}] (fpngrid3) -- (fpn2);
\draw [-{stealth[length=3mm]}] (fpn2) -- (fpngrid2);

\draw [-{stealth[length=3mm]}] (resgrid2) -- (fpn2);
\draw [-{stealth[length=3mm]}] (resgrid3) -- (fpn3);
\draw [-{stealth[length=3mm]}] (resgrid4) -- (fpn4);

%%% detection heads %%%
\node (head_vru) [right = 2.5 of fpngrid2, draw, rounded corners] {head ``VRU''};
\node (head_car) [below right = 0.4 and 2.5 of fpngrid3, draw, rounded corners] {head ``car-like''};
\node (head_vehicle) [above right = 0.4 and 2.5 of fpngrid3, draw, rounded corners] {head ``vehicle''};

\node (nms) [right = 2.0 of head_car, draw, rounded corners] {\rotatebox{90}{NMS}};
\node (obbs) [right = 0.8 of nms] {\rotatebox{90}{OBBs}};

\coordinate [right=1 of fpngrid3] (carveh_control);
\draw (fpngrid3) -- (carveh_control);
\draw [-{stealth[length=3mm]}, rounded corners=3pt] (carveh_control) |- (head_car);
\draw [-{stealth[length=3mm]}, rounded corners=3pt] (carveh_control) |- (head_vehicle);
\draw [-{stealth[length=3mm]}, rounded corners=3pt] (fpngrid2) -- (head_vru);
\draw [-{stealth[length=3mm]}, rounded corners=3pt] (head_vehicle) -| (nms);
\draw [-{stealth[length=3mm]}] (head_car) -- (nms);
\draw [-{stealth[length=3mm]}, rounded corners=3pt] (head_vru) -| (nms);
\draw [-{stealth[length=3mm]}] (nms) -- (obbs);

%%% detail for ResNet block %%%

\node (resnet_detail) [below left = 0.3 and 6.0 of res5, draw, dashed] {
\begin{tikzpicture}
\begin{scope}[local bounding box=res_main1, every node/.append style={
	yslant=0,xslant=1,solid},yslant=0,xslant=1,solid
]
\fill[white,fill opacity=0.9] (-.4,-.16) rectangle (.4,.16);
\draw[black,very thick](-.4,-.16) rectangle (.4,.16);%marking borders
\end{scope}
\node [below left = .35 and 1.3 of res_main1] {\footnotesize $1\times1$ conv, BN, ReLU};

\begin{scope}[local bounding box=res_main2,shift={($(res_main1.north)+(0,.5)$)}, every node/.append style={
	yslant=0,xslant=1,solid},yslant=0,xslant=1,solid
]
\fill[white,fill opacity=0.9] (-.4,-.16) rectangle (.4,.16);
\draw[black,very thick] (-.4,-.16) rectangle (.4,.16);%marking borders
\end{scope}
\node [below left = .35 and 1.3 of res_main2] {\footnotesize $3\times3$ conv, BN, ReLU};

\begin{scope}[local bounding box=res_main3,shift={($(res_main2.north)+(0,.5)$)}, every node/.append style={
	yslant=0,xslant=1,solid},yslant=0,xslant=1,solid
]
\fill[white,fill opacity=0.9] (-.4,-.16) rectangle (.4,.16);
\draw[black,very thick] (-.4,-.16) rectangle (.4,.16);%marking borders
\end{scope}
\node [below left = .35 and 1.3 of res_main3] {\footnotesize $1\times1$ conv, BN, ReLU};

\begin{scope}[local bounding box=res_bypass,shift={($(res_main2.east)+(1.0,0)$)}, every node/.append style={
	yslant=0,xslant=1,solid},yslant=0,xslant=1,solid
]
\fill[white,fill opacity=0.9] (-.4,-.16) rectangle (.4,.16);
\draw[black,very thick] (-.4,-.16) rectangle (.4,.16);%marking borders
\end{scope}
\node [below right = .35 and 1. of res_bypass] {\footnotesize $1\times1$ conv, BN};

\node (sum) [circle,inner sep=1pt, draw, solid, above right = .5 and .8 of res_main3] {+};
\coordinate [above= .3 of sum] (out);

\coordinate [below right= .3 and .8 of res_main1] (inwaypoint);
\coordinate [below = .3 of inwaypoint] (in);

\draw [rounded corners=3pt, solid,->] (in) -- (inwaypoint);
\draw [rounded corners=3pt, solid,->] (inwaypoint) -| (res_main1);
\draw [solid,->] (res_main1) -- (res_main2);
\draw [solid,->] (res_main2) -- (res_main3);
\draw [rounded corners=3pt, solid,->] (res_main3) |- (sum);
\draw [rounded corners=3pt, solid,->] (inwaypoint) -| (res_bypass);
\draw [rounded corners=3pt, solid,->] (res_bypass) |- (sum);
\draw [solid,->] (sum) -- (out);
\end{tikzpicture}
};
\draw [dashed] (res5_num.north west) -- (resnet_detail.north east);
\draw [dashed] (res5_num.south west) -- (resnet_detail.south east);

%%% detail for FPN block %%%
\node (fpn_detail) [above right = 0.5 and 3.0 of fpn4, draw, dashed] {
\begin{tikzpicture}
\node (sum) [circle,inner sep=1pt, draw, solid] {+};

\begin{scope}[local bounding box=transconv,shift={($(sum.north)+(0, .5)$)}, every node/.append style={
	yslant=0,xslant=1,solid},yslant=0,xslant=1,solid
]
\fill[white,fill opacity=0.9] (-.4,-.16) rectangle (.4,.16);
\draw[black,very thick] (-.4,-.16) rectangle (.4,.16);%marking borders
\end{scope}
\node [above left = .35 and .7 of transconv, text width= 7em] {\footnotesize $3\times3$\\[-1.5ex]transposed conv};

\begin{scope}[local bounding box=conv_short,shift={($(sum.west)+(-.8, 0)$)}, every node/.append style={
	yslant=.5,xslant=0,solid},yslant=.5,xslant=0,solid
]
\fill[white,fill opacity=0.9] (-.16,-.4) rectangle (.16,.4);
\draw[black,very thick] (-.16,-.4) rectangle (.16,.4);%marking borders
\end{scope}
\node [below = .6 of conv_short] {\footnotesize $1\times1$ conv};

\coordinate [left=1 of conv_short] (in_short);
\coordinate [above=.8 of transconv] (in_conv);
\coordinate [below=.8 of sum] (out);

\draw [solid,->] (in_short) -- (conv_short);
\draw [solid,->] (conv_short) -- (sum);
\draw [solid,->] (in_conv) -- (transconv);
\draw [solid,->] (in_short) -- (conv_short);
\draw [solid,->] (transconv) -- (sum);
\draw [solid,->] (sum) -- (out);

\end{tikzpicture}
};
\draw [dashed] (fpn4.north east) -- (fpn_detail.north west);
\draw [dashed] (fpn4.south east) -- (fpn_detail.south west);

\end{tikzpicture}

